Robust MIMO Detection using Hypernetworks with Learned Regularizers

Optimal symbol detection in multiple-input multiple-output (MIMO) systems is known to be an NP-hard problem. Recently, there has been a growing interest to get reasonably close to the optimal solution using neural networks while keeping the computational complexity in check. However, existing work based on deep learning shows that it is difficult to design a generic network that works well for a variety of channels. In this work, we propose a method that tries to strike a balance between symbol error rate (SER) performance and generality of channels. Our method is based on hypernetworks that generate the parameters of a neural network-based detector that works well on a specific channel. We propose a general framework by regularizing the training of the hypernetwork with some pre-trained instances of the channel-specific method. Through numerical experiments, we show that our proposed method yields high performance for a set of prespecified channel realizations while generalizing well to all channels drawn from a specific distribution.

==> figures/figures_old.tex <==
% \begin{figure}[t]
% 	\begin{tikzpicture}
% 		\draw[rounded corners, fill=blue, opacity = 0.1] (2.6, 0.25) rectangle (6.4, 0.75) {};
% 		\draw[rounded corners, fill=blue, opacity = 0.1] (2, -0.75) rectangle (7, -0.25) {};

% 		\node[] at (4.5, 0.5) {Hypernetwork: $g(\bbZ$;$\boldsymbol{{\Theta}})$};
% 		\node[] at (4.5, -0.5) {Main Network: $\Phi(\bbX, \ccalW)$};

		
% 		\draw[->] (1.5, -0.5) -- (2, -0.5);
% 		\draw[->] (7, -0.5) -- (7.5, -0.5);
% 		\node[] at (1, -0.5) {$\bbX$};
% 		\node[] at (8, -0.5) {$\bbY$};

% 		\draw[->] (2.2, 0.5) -- (2.6, 0.5);
% 		\draw[->] (6.4, 0.5) -- (6.8, 0.5);		
% 		\node[] at (2, 0.5) {$\bbZ$};
% 		\node[] at (8.2, 0.5) {{\scriptsize$\underbrace{[\bbw_{(0)},\bbw_{(1)},\cdots, \bbw_{\text{\tiny{(L-1)}}}]}_{}$}};
		
% 		\draw [->] (8.2, 0.4) to [out=-150,in=30] (4.5, -0.25);
% 	\end{tikzpicture}
% 	\caption{The general scheme of a hypernetwork. The hypernetwork $g(.)$ takes the input $\bbZ$ and generates the weights $\bbW$, which are fed into the main network. Then, the main network $\Phi(.)$ takes as input $\bbA$ and returns the output $\bbB$. \red{Make the output of the hypernetwork be $\bbW$ instead of those $L$ vectors. Also, update $\ccalW$ to $\bbW$ and all the other symbols.}}
% 	\label{fig:hyperNet}
% \end{figure}
